Hang With Your Buddies to Resist Intersection Attacks

Some anonymity schemes might in principle protect users from pervasive network surveillance - but only if all messages are independent and unlinkable. Users in practice often need pseudonymity - sending messages intentionally linkable to each other but not to the sender - but pseudonymity in dynamic networks exposes users to intersection attacks. We present Buddies, the first systematic design for intersection attack resistance in practical anonymity systems. Buddies groups users dynamically into buddy sets, controlling message transmission to make buddies within a set behaviorally indistinguishable under traffic analysis. To manage the inevitable tradeoffs between anonymity guarantees and communication responsiveness, Buddies enables users to select independent attack mitigation policies for each pseudonym. Using trace-based simulations and a working prototype, we find that Buddies can guarantee non-trivial anonymity set sizes in realistic chat/microblogging scenarios, for both short-lived and long-lived pseudonyms.

==> analysis.tex <==
\section{Security Analysis}

\app makes three guarantees with respect to anonymity sets.
The first one follows from the proactive approach while
the two later follow from the reactive approach.

\begin{enumerate}
\item Each member $i$ will maintain a minimum anonymity set of size $B$, where $B$ is
the size of the buddy set member $i$ belongs to.
\item Each member $i$ will maintain its member anonymity $\textsc{UserAnon}_{i,t} \geq R$, 
where $R$ is the desired size of the set, at any given round $t$.
\item Each pseudonym $j$ will maintain a pseudonym anonymity $\textsc{NymAnon}_{j,t} \geq R$
at any given round $t$.
\end{enumerate}

\subsection{Proactive Approach}

\app guarantees that each member will always maintain a certain minimum anonymity
set. The size of this set is defined by the size of the buddy set a particular 
member belongs to. Therefore, if the buddy set consists of $B$ members, 
then each member of this set is indistinguishable from $B-1$ members, hence,
he ``hides" among $B$ other members or more formally, 
he maintains an anonymity set of $B$ members.  
\app achieves this guarantee by forcing all members of the same buddy set
to behave identically. More specifically, during each round $t$ member $i$'s
cleartext message is published only if every other member $j$ from $i$'s buddy
set is active as well. Following this approach, each member of the buddy set 
appears to be an owner of $B$ pseudonyms at the minimum. 
This is easy to see as one active member always implies one active pseudonym
and there are $B$ such members, in addition to members from other buddy sets who 
coincidentally exhibit the same behavior. 
Additionally, because of the symmetry of actions of members and pseudonyms,
each pseudonym appears to be owned by $B$ members at the minimum. 

One caveat exists in the above analysis, however. So far we were able to assume 
that the minimum anonymity set is equal to $B$ because we ignored the existence of dishonest
members colluding with the adversary. Even though the behavior of honest and dishonest
members within the same buddy set would be the same, they can claim their pseudonym
thereby reducing the anonymity set of honest members to $B-f$, where $f$ is the number
of dishonest members in the buddy set. The probability of a buddy set containing
a dishonest member depends on $f$ and a particular grouping mechanisms \app uses
(e.g., random selection, by offline time). In case of a random buddy set construction,
we can expect $\lfloor \frac{f}{\frac{N}{K}} \rfloor$ %eh, really helpful
dishonest members per buddy set. 

\subsection{Reactive Approach}

Buddies achieves the minimum anonymity set guarantee by solely analyzing
and adjusting the behavior of members of the same buddy set.
However, maintaining a large buddy set, while desirable, is very inefficient
because all members must be active during the same round, which is 
one out of $s^n$ states a group potentially can be in, where
$n$ is the buddy set size and $s$ is the number of 
member's states (e.g., offline, online-inactive, online-active).

Fortunately, the actual anonymity set of a particular member might be, 
and most likely is, much greater than the minimum buddy-anonymity 
set because some of the other members are likely to exhibit the same behavior,
and through proper choices that anonymity set can be preserved 
at a desired level.
The reactive approach builds upon this observation and uses anonymity meters
allowing to calculate and maintain the larger anonymity sets for members. 

\app uses two anonymity meters $\textsc{UserAnon}_{i,t}$ and 
$\textsc{NymAnon}_{j,t}$ to calculate the effective 
anonymity sets as defined by the member and pseudonym anonymity.

\emph{Member anonymity.} We say that a member $i$ remains anonymous 
if $\forall i \in \mathbb{U}, \textsc{UserAnon}_{i,t} \ge R$.

\app achieves this guarantee by ...

\emph{Pseudonym anonymity.} We say that a pseudonym $j$ remains
anonymous
if $\forall j \in \mathbb{P}, \textsc{NymAnon}_{j,t} \ge R$.

\app achieves this guarantee by ...


The above two guarantees lead to a couple of observations. 
\begin{enumerate}
\item A member $i$ who participates in every round $t$ will maintain 
$\textsc{UserAnon}_{i,t} = \mathbb{P}$, the maximum level 
of member anonymity.
At round $t=0$, $i$'s member anonymity set contains every pseudonym.
If $i$ participates in every round $t$ ($i \in \mathcal{O}_t$), 
then there is never a pseudonym removed from this set, regardless
of the state of $\mathcal{A}_t$, because the fact that $i$ is online 
makes him appear as a potential owner of all currently active pseudonyms
in $\mathcal{A}_t$.

\item Member $i$'s pseudonym will always contain $i$ in its pseudonym
anonymity set. 

\item An always active pseudonym may eventually be squelched to maintain 
his anonymity. 

\item ...
\end{enumerate}


\subsection{Others}
The security guarantees provided by \app
effectively reduce into keeping proper count.
With respect to the grouping schemes,

Grouping states which to analyze:
\begin{enumerate}
  \item state in which groups have already been formed -- straight forward
  \item dynamic with all online -- go offline join a group, if only K to 2 * K - 1 peers remain form a final group
  \item dynamic with all offline -- queue to get online
  \item dynamic with enough in both -- derive directly from all online / all offline
  \item dynamic with not enough in online -- we queue them up and wait for them to get online
  \item dynamic with not enough in offline -- they never get online or we force queue the bottom members of the online group with them
\end{enumerate}

Alternative approach analysis:
\begin{enumerate}
  \item anonymity sets are already maxed out or minimum anonymity equals group size -- nothing, this is handled by the above
  \item sets are defined -- then we can toss out messages for users in offline groups
  \item sets must be fixed, i.e., they form groups
  \item sets are not fixed, i.e., we obey minimal anonymity but there are no real groups.
\end{enumerate}

In this section,
we examine the guarantees promised by \app:
\begin{enumerate}
  \item a nym will maintain a minimum level of anonymity
  \item an always present individual will remain in all nym anonymity sets
  \item an always active nym may eventually be squelched to maintain his anonymity
  \item a one-to-one member:nym mapping can result in members being unconditionally being squelched whereas a one-to-many does not
  \item a one-to-many system allows continual messages without requiring a halt
  \item \app will delay in an effort to keep around higher utility peers
  \item the fixed output system can make progress where the basic approach can without invalidating these guarantees
\end{enumerate}

